Mapping Tractography Across Subjects

Diffusion magnetic resonance imaging (dMRI) and tractography provide means to study the anatomical structures within the white matter of the brain. When studying tractography data across subjects, it is usually necessary to align, i.e. to register, tractographies together. This registration step is most often performed by applying the transformation resulting from the registration of other volumetric images (T1, FA). In contrast with registration methods that "transform" tractographies, in this work, we try to find which streamline in one tractography correspond to which streamline in the other tractography, without any transformation. In other words, we try to find a "mapping" between the tractographies. We propose a graph-based solution for the tractography mapping problem and we explain similarities and differences with the related well-known graph matching problem. Specifically, we define a loss function based on the pairwise streamline distance and reformulate the mapping problem as combinatorial optimization of that loss function. We show preliminary promising results where we compare the proposed method, implemented with simulated annealing, against a standard registration techniques in a task of segmentation of the corticospinal tract.

==> materials.tex <==
%\section{Materials}
%\label{sec:materials}
The dataset in our experiments was recorded with a $3T$ scanner at Utah Brain Institute\footnote{The authors are grateful to Prof. Mark B.Bromberg, Prof. Lubdha Shah and Prof. Perry Renshaw of the Department of Neurology and the Department of Radiology, University of Utah (US), for their assistance in acquiring MR data},
$65$ gradients ($64$ + $b0$); b-value = $1000$; anatomical scan ($2\times2\times2mm^3$). We reconstructed the streamlines using EuDX tracking algorithm%~\cite{garyfallidis2012towards} 
from dipy\footnote{\url{http://www.dipy.org}}. CST data was manually segmented by experts\footnote{The authors thank doctor Nivedita Agarwal of Radiology Unit, S.Maria del Carmine Hospital, Rovereto, Italy, for manually segmenting the CST} using the computer aided tractography segmentation software tool~\cite{olivetti2013fast}. 
The dataset contained $4$ CST-left plus $4$ CST-right of healthy controls.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mlini2014_mapping"
%%% End: 

